A wind-blown bubble in the Central Molecular Zone cloud G0.253+0.016

G0.253+0.016, commonly referred to as "the Brick" and located within the Central Molecular Zone, is one of the densest ($\approx10^{3-4}$ cm$^{-3}$) molecular clouds in the Galaxy to lack signatures of widespread star formation. We set out to constrain the origins of an arc-shaped molecular line emission feature located within the cloud. We determine that the arc, centred on $\{l_{0},b_{0}\}=\{0.248^{\circ}, 0.18^{\circ}\}$, has a radius of $1.3$ pc and kinematics indicative of the presence of a shell expanding at $5.2^{+2.7}_{-1.9}$ km s$^{-1}$. Extended radio continuum emission fills the arc cavity and recombination line emission peaks at a similar velocity to the arc, implying that the molecular and ionised gas are physically related. The inferred Lyman continuum photon rate is $N_{\rm LyC}=10^{46.0}-10^{47.9}$ photons s$^{-1}$, consistent with a star of spectral type B1-O8.5, corresponding to a mass of $\approx12-20$ M$_{\odot}$. We explore two scenarios for the origin of the arc: i) a partial shell swept up by the wind of an interloper high-mass star; ii) a partial shell swept up by stellar feedback resulting from in-situ star formation. We favour the latter scenario, finding reasonable (factor of a few) agreement between its morphology, dynamics, and energetics and those predicted for an expanding bubble driven by the wind from a high-mass star. The immediate implication is that G0.253+0.016 may not be as quiescent as is commonly accepted. We speculate that the cloud may have produced a $\lesssim10^{3}$ M$_{\odot}$ star cluster $\gtrsim0.4$ Myr ago, and demonstrate that the high-extinction and stellar crowding observed towards G0.253+0.016 may help to obscure such a star cluster from detection.

==> figures/extinction.tex <==
\begin{figure*}
\begin{center}
\includegraphics[trim = 0mm 20mm 0mm 20mm, clip, width = 0.98\textwidth]{figures/extinction_comp.pdf}
\end{center}
\caption{Molecular hydrogen column density, and extinction maps at various wavelengths towards \brick. The grey and black contours indicate 1\,mag and 10\,mag of extinction at the respective wavelengths.}
\label{Figure:ext}
\end{figure*}

==> figures/figure_large-scale_vel.tex <==
\begin{figure*}
\begin{center}
\includegraphics[trim = 20mm 15mm 20mm 30mm, clip, width = 0.98\textwidth]{figures/arc_large-scale_vel.pdf}
\end{center}
\caption{Left: The velocity field of the arc's parent sub-cloud. Right: The modelled velocity field. All symbols are identical to those presented in Figure~\ref{Figure:arc_LS}.}
\label{Figure:arc_LS_vel}
\end{figure*}
